LiDiTE: a Full-Fledged and Featherweight Digital Twin Framework

The rising of the Cyber-Physical System (CPS) and the Industry 4.0 paradigms demands the design and the implementation of Digital Twin Frameworks (DTFs) that may support the quick build of reliable Digital Twins (DTs) for experimental and testing purposes. Most of the current DTF proposals allow generating DTs at a good pace but affect generality, scalability, portability, and completeness. As a consequence, current DTF are mostly domain-specific and hardly span several application domains (e.g., from simple IoT deployments to the modeling of complex critical infrastructures). Furthermore, the generated DTs often requires a high amount of computational resource to run. In this paper, we present LiDiTE, a novel DTF that overcomes the previous limitations by, on the one hand, supporting the building of general-purpose DTs at a fine-grained level, but, on the other hand, with a reduced resource footprint w.r.t. the current state of the art. We show the characteristics of the LiDiTE by building the DT of a complex and real critical infrastructure (i.e., the Smart Poligeneration Microgrid of the Savona Campus) and evaluating its resource consumption. The source code of LiDiTE, as well as the experimental dataset, is publicly available.

==> background.tex <==
\section{Background}
\label{sec:background}

%\gcnote{Lasciamolo per dopo perché dipende dal contenuto del paper}

%\ernote{mettere qualcosa su docker networking...}

% \subsection{Enterprise and industrial networks}
% \label{sec:industrial}

% \ernote{per questa parte ci siamo ispirati al purdue model e IEC62443, defence in depth vedi anche \url{https://cms-cdn.selinc.com/assets/Literature/Publications/Technical\%20Papers/6917_CompleteIEC61850_DD_20190703_Web.pdf?v=20190703-230520}}. 
% \gcnote{io qui partirei dagli standard che abbiamo visto}
% \gcnote{Fig. 2 forse non serve}

    % \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{fig/schema.png}
%     \caption{General structure of an industrial network.}
%     \label{fig:schema}
% \end{figure}

\subsection{Virtualization and containerization}
\label{sec:virt}
%\ernote{Verficare se in sez. V ci sono cose da spostare qui e duplicate (vedi KVM ref)}
Virtualization and containerization are the two most widely used solutions to host isolated applications in a single computer system.

Virtualization partitions a single physical server into several Virtual Machines (VM).
A VM creates a virtual version of each computer capability (e.g., processor, storage, or network) and can run different operating systems and applications while sharing the physical resources of the server.
Virtualization leverages a specific software layer, namely the \emph{hypervisor}.

Containerization is a lightweight alternative to virtualization.
This solution involves encapsulating an application and its dependencies within a container, i.e., its own isolated environment.
Containers share both the physical resources and the same operating system of the hosting server.
Containerization is enabled through the underlying host operating system kernel.

Two of the most commonly used solutions to implement virtualization and containerization are \emph{Linux Kernel-based Virtual Machine} (KVM)~\cite{goto2011kernel} and \emph{Docker}~\cite{docker21}, respectively.

KVM is a virtualization solution for Linux and can host multiple virtual machines running unmodified Linux or Windows images.
Instead, Docker can run on top of both Windows and Linux hosts.
Notice that, in this paper, we refer to Linux Docker.
Consequently, we must consider each container only able to run Linux applications as an isolated process of the hosting system.

\subsection{Docker networking}
\label{sec:dockernet}
Docker's networking allows containers to connect together or connects them to non-Docker workloads. 
In particular, the core networking functionalities are implemented through drivers, using a pluggable architecture.
From the point of view of a container, the configured driver is transparent.
%\glnote{(unless \texttt{network\_mode: none} has been specified)}
This means that a container (unless networking is explicitly disabled) always has a network interface that is configured and operates as if it were a physical host.
%\ernote{forse bisgona mitigare always per il fatto che esiste network none}. 
Instead, each driver establishes how a container can interact with the host and other network nodes.

Docker provides different built-in drivers~\cite{dockernet21} and the most commonly used are \emph{host}, \emph{bridge}, and \emph{macvlan}.

\begin{figure}
    \centering
    \includegraphics[width=0.75\columnwidth]{fig/docker network.png}
    %\includesvg[width=0.8\columnwidth]{fig/docker network.svg}
    \caption{An example of an host executing Docker containers.}
    \label{fig:dockerdrvs}
\end{figure}

To highlight the difference between each driver, consider as an example the host depicted in Figure~\ref{fig:dockerdrvs}.
It has a physical adapter \emph{eth0} that connects it to a physical network and run six containers C$_1$\dots C$_6$.

C$_1$ is configured with the host driver that allows the container to use the host’s networking directly. 
This means that C$_1$ runs without any network isolation and inherits the configuration (e.g, the IP address 198.51.100.15) and all the capabilities of the hosting system.

The bridge driver represents the default solution for creating virtual networks and connecting containers that need to communicate.
In the example, the host is configured with two bridge network, i.e., \emph{bridge\_network1} and \emph{bridge\_network2}. 
To each bridge network is associated a host bridge interface (e.g., \emph{br1} is associated with \emph{bridge\_network1}) and an IP class (e.g., 172.16.10.0/24 is associated with \emph{bridge\_network1}).
The first IP address of the associated class is always assigned to the host using the bridge interface (e.g., 172.16.10.1 is assigned to the host \emph{br0} interface).
Docker automatically assigns to each connected container an unallocated IP address and configure their default gateway with the address of the bridge interface.
As a result, the host always works as the default router of all bridge networks.
Notice that Docker enforces isolation for bridge networks allowing communication only between containers that are connected to the same bridge.
For example, C$_2$,  C$_3$, and C$_4$ are configured with the bridge driver.
For this reason, C$_3$ can communicate with C$_4$ but not with C$_2$.
Nevertheless, all the three containers con communicate with nodes that are reachable through non-bridge networks, e.g., containers C$_1$, C$_5$, and C$_6$.

Finally, the macvlan driver leverages a Linux kernel module that enables creating multiple virtual interfaces on top of a single host's network interface.
This configuration makes a container appearing to be a physical device directly connected to the network associated to the macvlan interface.
Unlike a bridge network, the Linux kernel module implementing a macvlan enforces isolation between containers and the host, i.e., filters the traffic between macvlan interfaces and the host itself.
For this reason, Docker assigns an unused IP address to a container that uses a macvlan, but the default gateway address must be explicitly configured to point to a node different from the host.
In the example, C$_5$ and C$_6$ are configured with the macvlan driver on top of the eth0 interface.
They look directly connected to the physical network and have configured an address of the same class and with the same default gateway as the host interface (e.g., C$_5$ is configured with the IP address 198.51.100.20). 
%\gcnote{orchestrators}
\subsection{Docker Compose}
\label{sec:dockercompose}
%\glnote{o orchestrator}
\ernote{TBD}

==> bio.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> usecase.tex <==
\section{Use Case}
\label{sec:usecase}

In this section we introduce our use case which will also serve as working example throughout the rest of the paper.

\subsection{Overview}

\begin{figure}[t]
     \centering
     \includegraphics[width=\columnwidth]{fig/spm.png}
     \caption{A schematic representation of the SPM infrastructures.}
     \label{fig:spm}
\end{figure}

The Smart Polygeneration Microgrid (SPM)~\cite{spm} is a power generation plant deployed within the Savona campus of the University of Genoa.
The campus hosts a number of facilities for university students and staff, including a gym and a tennis court.
Classrooms, laboratories and offices are located inside five buildings.
Moreover, a sixth building contains the library and some study rooms.
In general, the SPM builds on top of three distinct, yet interconnected, infrastructures, i.e., the university campus, the ICT network and the energy system (see Figure~\ref{fig:spm}).
These infrastructures host several subsystems.
Below, we provide a detailed description of those that are relevant in this paper.

\subsection{Power plant}

The structure of the microgrid is that of a power ring, connecting all the subsystems.
The main power generation subsystem amounts to a solar plant installed on the roof of building B. 
Solar panels can output up to 80.64 kW~\cite{Bracco17smart}, depending on environmental factors, such as season, daytime and weather conditions.
If needed, a Capstone\textsuperscript{\textregistered} C65~\cite[\S 4.1]{bracco-gas-turbine}
%\footnote{\url{https://www.capstoneturbine.com/products/c65}}
gas turbine can be activated to integrate the energy production.
The turbine is a co-generative system, combining combustion and heat, which produces 65 kW.
Furthermore, an energy storage is recharged to accumulate energy surplus and, alternatively, discharged to cover energy deficit.
The overall energy demand amounts to the sum of the demands of each building, which depend on the local energy consumption.
Finally, in case of excess of demand, the SPM drains from the public energy distribution network.
The overall structure is depicted in Figure~\ref{fig:physical}.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/physical.png}
    \caption{The SPM power ring}
    \label{fig:physical}
\end{figure}

\subsection{On field controllers}

Each subsystem is under the control of a field device.
Field devices are connected to the central SCADA system (see Section~\ref{sec:scada}).
Field controllers feed the SCADA server with data from their own subsystem, e.g., the currently produced power, and receive commands to be applied, e.g., to switch on and off the subsystem.
Communications are implemented in two ways.
Buildings' cabinets are directly connected with the SCADA server through Modbus/TCP~\cite{swales1999open}. %\gcnote{add ref?}.
Instead, storage, turbine and solar controllers interact using the Publish/Subscribe pattern.
%are connected via MQTT\gcnote{add ref?}.\ernote{da rivedere..secondo me se ci riferiamo a Ditto non usa MQTT..meglio mettere paradigma pub/sub, https://www.eclipse.org/ditto/connectivity-overview.html protocolli supportati}
The connection occurs through a message broker server which handles the message queue between the field devices and the SCADA server.
The SCADA server relies on REST APIs to query the broker.
The overall schema is depicted in Figure~\ref{fig:field}.
\gcnote{questa figura è proprio brutta...}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/field_new.png}
    \caption{Field devices communication structure}
    \label{fig:field}
\end{figure}

\subsection{Campus network}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{fig/network.png}
    \caption{ICT network scheme}
    \label{fig:network}
\end{figure*}

The campus ICT infrastructure consists of a segmented enterprise network (see Figure~\ref{fig:network})\ernote{direi di cambiare i nomi nella figura}\gcnote{per me ok}.
The four main segments are called \emph{client}, \emph{DMZ}, \emph{control}, and \emph{field}.
The client network hosts personal devices belonging to staff and students, and it is accessible throughout the entire campus.
The DMZ network is for campus servers located inside the server room, and it is meant to expose remotely accessible, public services.
The control network hosts servers and workstations dedicated to the smart grid management.
The field network hosts the field devices.
Finally, the campus is connected to the Internet through an Internet Service Provider (ISP) router.
The overall segmentation is enabled by three firewalls that allow each network to operate under distinct security policies.
For example, a policy enforced on the field firewall denies field devices to browse the Internet and only allows incoming connections from the control network.
\gcnote{rifrasta}

\subsection{Energy Management System}

The Energy Management System (EMS) is a centralized, automatic control process that handles the SPM power generation logic.
The goal of the EMS is to employ the power generation subsystems so to maximize the SPM efficiency in terms of costs and ecological footprint.\gcnote{check}
To this aim, the EMS monitors the internal demand and the overall power generation.
If possible, solar energy generation is privileged since it comes at almost no cost and has negligible effects on the environment.
When solar production exceeds the demand, the energy surplus is redirected to the energy storage.
To do this, the EMS activates the \emph{charge} mode of the energy storage.
If the energy storage cannot switch to charge mode, e.g., because full charge has been reached, the surplus is dissipated.
When the solar production is insufficient, the EMS attempts to cover the energy deficit by executing the following steps.
\begin{enumerate}
    \item[1.] The energy storage is set to \emph{discharge} mode.
    \item[2.] If 1. is unfeasible, the gas turbine is started.
    \item[3.] If 2. is unfeasible or uneconomical, energy is bought from the public supplier. 
\end{enumerate}

\subsection{SCADA system}
\label{sec:scada}

The SPM is under the scope of a SCADA system.
The SCADA system acquires data from the peripheral subsystems and allows operators for monitoring the SPM.
Furthermore, operators can manually instruct the SPM, by modifying the state of the system.
The SCADA system runs on the SCADA server (see above) and operators access its interface through a dedicated workstation inside the SPM control room.

\subsection{Campus staff and students}

Mainly two categories of people move inside the campus, i.e., staff members and students.
Staff members include SPM operators, teaching and administrative personnel.
Both students and staff members can connect to the SPM enterprise network with their client devices, e.g., laptops.
The number of people inside the campus varies depending on some factors such as the daytime and the period of the year.
% \gcnote{non bellissimo, ma dipende da quello che vogliamo scrivere dopo}

% \subsection{Infrastructure description}

% \gcnote{da rischivere da qui in giù}
% The use case infrastructure is organized according to Figure~\ref{fig:schema}.
% Each of the four zones is implemented by a sub-network which hosts the devices belonging to that zone.
% In particular:
% \begin{itemize}
%     \item greenhouse equipment, i.e., sensors and actuators, is connected to the \emph{industrial} network;
%     \item industrial control devices, i.e., workstations and SCADA server, are connected to the \emph{industrial/enterprise} network;
%     \item business-related services, i.e., CRM and ERP, as well as the laptop, are connected to the \emph{enterprise} network, and;
%     \item public services, i.e., DNS, mail and web, stay under the \emph{dmz} network.
% \end{itemize}

% \gcnote{organzzazione dei plc: vogliamo dire qualcosa sul fatto che sono connessi via Modbus/TCP?}

% \gcnote{regole di accesso}
% In order to prevent undesired interactions, network connectivity is restricted by access policies.
% In particular, the network is organized according to four nested security zones.
% Three firewalls are in charge for enforcing the security policy of each zone.
% We describe them below.
% \gcnote{Enrico, qui devi completare tu}
% \begin{itemize}
%     \item \emph{Perimeter firewall}.
%     \item \emph{Enterprise firewall}.
%     \item \emph{Industrial firewall}.
% \end{itemize}

